An Algebraic Approach for Reasoning About Information Flow

This paper concerns the analysis of information leaks in security systems. We address the problem of specifying and analyzing large systems in the (standard) channel model used in quantitative information flow (QIF). We propose several operators which match typical interactions between system components. We explore their algebraic properties with respect to the security-preserving refinement relation defined by Alvim et al. and McIver et al. We show how the algebra can be used to simplify large system specifications in order to facilitate the computation of information leakage bounds. We demonstrate our results on the specification and analysis of the Crowds Protocol. Finally, we use the algebra to justify a new algorithm to compute leakage bounds for this protocol.

==> analyses.tex <==
\commentAA{The structure of this section will be changed a little bit this Tuesday. The graphs have been changed already, so the text and captions may be a little bit off}

We now analyze the information-leakage of the channels obtained for all variations 
of each protocol, in the light of the capacities defined in Section~\ref{sec:prelqif}.
Recall that the smaller the capacity of a channel, the less information 
an adversary will obtain about the secret by observing the output of that channel, 
and the safer, hence, the channel is considered.

\subsection{\label{sec:analdin} Analyses of the Dining Cryptographers}

We implemented both variations of the Dining cryptographers for 
5, 6, 7, 8, and 9 cryptographers. 
Our results suggest the complete-DC variation is safer than the cycle-DC variation, 
yielding smaller values for all capacities measured.

\subsubsection{Results for multiplicative capacities%
% $\mathcal{L}_\forall\hyperc{\pi}{C}$ and $\mathcal{L}_\forall\hyperc{\forall}{C}$
.}

It has been proven \cite{addmult} that the multiplicative capacity
$\mathcal{L}_\forall\hyperc{\pi}{C}$ (which quantifies over all gain-functions $g$ for
a fixed prior $\pi$) collapses into the multiplicative capacity $\mathcal{L}_\forall\hyperc{\forall}{C}$ (which quantifies over all priors and gain-functions). 
Since we consider any cryptographer can be the payer (and the prior must, hence,
have full support), we focus only on the latter capacity, which is easy to compute
thanks to the following result.

\begin{Theorem}[\cite{capacity}]
\label{capacity}
Given channel $C{:}\calx{\times}\caly{\rightarrow}\reals$,
$\mathcal{L}_\forall\hyperc{\forall}{C}{=}\log \sum_{y \in \caly}\max\limits_{x \in \calx} C(x,y).$
\end{Theorem}

Figure~\ref{figure:mlcdin}, 
\commentA{I have no idea why this figure looks that bad. Gonna fix that later. Probably use some better tool for making graphs (suggestions are more than welcome :) )}
shows the values of this capacity for both variants of the DC protocol, 
and varying values of the probability $p$ of heads. 
Note that, since the protocol always reveals whether one of the cryptographers is paying, 
the minimum capacity is 1,
\commentM{Capacity is 1 because Theorem~\ref{capacity} says it coincides with
min-capacity.
Should we interpret this result here?} which is achieved when $p=0.5$. 
In this scenario, no information regarding the payer leaked.
\commentM{Also, the $x$-axes start from 0.5. We have to explain why
(because capacity is symmetric w.r.t. that value).}

It is clear from the graph that the complete variation leaks less than the cycle one. 
Also, while the capacity of the cycle variation increases rapidly even when $p$ approaches
$0.5$, the complete variation is less susceptible to these small changes, 
keeping the information leakage about the payer at almost 0.


\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{figures/dining.png}
\caption{Values of $\mathcal{L}_\forall\hyperc{\forall}{C}$
$\mathcal{L}^+_\forall\hyperc{\pi_u}{C}$ for both variations of the Dining Cryptographers with vaying number of cryptographers, and different values of probabilities of heads. }
\label{figure:mlcdin}
\end{figure}

\subsubsection{Results for additive capacity%
%$\mathcal{L}^+_\forall\hyperc{\pi}{C}$
.}
The additive capacity $\mathcal{L}^+_\forall\hyperc{\pi}{C}$ (quantifying
over all gain functions $g$, for a given prior $\pi$) can be
computed as follows 
$ 
\mathcal{L}^+_\forall\hyperc{\pi}{C}=\sum_{x,y} \pi(x) |C(x,y) - \sum_{x'}\pi(x')C(x',y)|
$
~\cite{addmult}.
Note that, unlike its multiplicative counterpart, this capacity actually depends on $\pi$. 

Figure~\ref{figure:mlcdin} shows the values for this capacity for an uniform prior, 
\commentA{This is quite dull. Any suggestions of other priors?} 
and varying probabilities $p$ of heads. 
Again, we see that the complete variation is more secure than the cycle one, 
and its capacity keeps almost unaltered until $p$ deviates substantially from $0.5$.

\subsection{Analyses of Crowds}

We implemented both variants of the Crowds protocol for 9 and 16 users, 
and from 1 up to 3 corrupted users. 
In the grid variation, we need to consider another variable: the position 
of the corrupt users makes a great difference in the channels' capacities. 
\commentM{Giving an intuition of why this difference happens is important.
Say a couple of sentences about it.}
We considered all the different possible positions, up to symmetry.

\subsubsection{Results for multiplicative capacities%
%$\mathcal{L}_\forall\hyperc{\pi}{C}$ and $\mathcal{L}_\forall\hyperc{\forall}{C}$
.}

We again used theorem~\ref{capacity} to calculate $\mathcal{L}_\forall\hyperc{\forall}{C}$. 
Figure~\ref{figure:mlccr} shows the corresponding values for 9 users and for 16 users.
It is very interesting to notice that, in the regular protocol, the probability $p_f$ 
of forwarding does not change the capacity 
\commentA{Is the capacity supposed to not vary in relation to $p_f$? 
I was not expecting this}
\replyM{Yes, it is expected! We should give a reference to a study that shows why.
Kostas has some paper on this, and I think Geoffrey too.}, 
but it does for the grid variation.
As we can see, the capacities of the channels on the grid variation varies considerably 
according to the position of the corrupt users.

For some choices of corrupt users positions, the grid variation actually seems to be safer 
than the regular one. 
This seems to happen when corrupt users are close to each other, and cannot interact 
directly with many honest users.
\commentA{I have the positions as well. If it is interesting, we can make a deeper 
analysis on that}

\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{figures/crowds.png}
\caption{Values of $\mathcal{L}_\forall\hyperc{\forall}{C}$
$\mathcal{L}^+_\forall\hyperc{\pi_u}{C}$ for both variations of the Crowds with vaying number of corrupt users, and different values of probabilities of forwarding the request. }
\label{figure:mlccr}
\end{figure}

\subsubsection{Results for additive capacity%
%$\mathcal{L}^+_\forall\hyperc{\pi}{C}$
.}

We again use the equation on section~\ref{sec:analdin} to compute 
$\mathcal{L}^+_\forall\hyperc{\pi}{C}$. 
We use the same channels as before, and a uniform prior. 
Figure~\ref{figure:mlccr} shows the results.

We can see that the additive capacities behave differently from the multiplicative ones. For instance, in no instance the additive capacity of the grid variation on 16 users was lower than the regular one, which did not happen regarding the multiplicative ones, as can be seen in Figure \ref{figure:mlccr}. 


